cp3-bench: A tool for benchmarking symbolic regression algorithms tested with cosmology

We introduce cp3-bench, a tool for comparing symbolic regression algorithms which we make publicly available at https://github.com/CP3-Origins/cp3-bench. Currently, cp3-bench includes 12 symbolic regression algorithms which can be automatically installed as part of cp3-bench. The philosophy behind cp3-bench is that it should be as user-friendly as possible, available in a ready-to-use format, and allow for easy additions of new algorithms and datasets. Our hope is that users of symbolic regression algorithms can use cp3-bench to easily install and compare symbolic regression algorithms to better decide which algorithms to use for their specific tasks at hand. To introduce and motivate the use of cp3-bench we present a benchmark of 12 symbolic regression algorithms applied to 28 datasets representing six different astrophysical setups. Overall, we find that most of the benched algorithms do poorly in the benchmark and suggest possible ways to proceed with developing algorithms that will be better at identifying ground truth expressions for cosmological datasets. Our demonstration benchmark studies the significance of dimensionality of the feature space and precision of datasets. We find both to be highly important for symbolic regression tasks to be successful. On the other hand, we find no indication that inter-dependence of features in datasets is important, i.e. it is not in general a hindrance for symbolic regression algorithms if datasets e.g. contain both $z$ and $H(z)$ as features. Lastly, we find no indication that performance of algorithms on standardized datasets are good indicators of performance on particular astrophysical datasets. This suggests that it is not necessarily prudent to choose symbolic regression algorithms based on their performance on standardized data. A more robust approach is to consider a variety of algorithms, chosen based on the particular task at hand.

==> grid.tex <==
We should set hyperparameters (and possibly grids) to make each algorithm set for maximal chance of success and at the same time remember to set parameters equally (i.e. number of iterations should be the same for all agorithms we can set it).


ITEA (1902.03983)
User-defined parameters incl grid choice made in their comparison:

[Mutation]
exponents      = {(-3, 3), (-2,2)}
termlimit      = (2,15)
nonzeroexps    = 10
transfunctions = [Id, Sin, Cos, SqrtAbs, Log, Exp] #Sofie removed Tanh
measures       = ["RMSE", "NMSE", "MAE", "R^2"]

[Algorithm]
npop      = {100,250,500}
ngens     = 1e5/npop
algorithm = ITEA

[Constraints]
penalty = NoPenalty
shapes  = []
domains = Nothing

QLattice  (https://www.biorxiv.org/content/10.1101/2022.01.14.475226v3.full)
User-defined parameters incl grid choice made in their comparison:

I appears that the only hyper-parameter to vary in this algorithm is
n_epochs. We could here choose a grid of {1e5/100, 1e5/250, 1e5/500}



gpzgd (don't have access to their paper!)
From their gecco2022 competition configureation (form their github page), we see
pop_size=200
generations=250
min_tree_init=2
max_tree_init=4
crossover_rate=0.3
point_mutation_rate=0.3
sub_mutation_rate=0.4
max_tree_depth=-1
max_tree_nodes=50
tournament_size=3
elitism_rate=1
mutation_sigma=0.1
standardise=Y
opset=ADD,SUB,MUL,SIN,ERC,VAR
coef_op=Y
learning_rate=0.01
learning_epochs=3


GeneticEngine (their papers suck for our purpose -- they don't explain hyperparameter choices)
Looking around in GeneticEngine/examples/regression_XXX.py on their github page, I'd say we should set something along the lines of

Functions: [Plus, Mul, SafeDiv, Literal, Var, SafeSqrt, Sin, Tanh, Exp, SafeLog]

Number of generations: {1e5/100, 1e5/250, 1e5/500}

Choose MSE as the fitness function.
In addition, in regression.py they make the following choices:

probability_crossover=0.75,
probability_mutation=0.01,
number_of_generations=50,
max_depth=10,
population_size=200,
selection_method=("tournament", 2),
n_elites=5,



PySR
Custom loss function: Choose mse
Based on their example using "as many PySR features as possible" on github (but values changed to fit with choices we make for algorithms above):

population size: 200
ncyclesperiteration: 500
niterations: Set to reasonable or number or let it run "forever" with stopping criteria based on functions not getting better or spent more than, say, 24 hours

maxsize = 12
maxdepth = 3 (we don't want nesting)
    binary_operators=["*", "+", "-", "/"],
    unary_operators=["square", "cube", "exp", "cos2(x)=cos(x)^2"],
    constraints={
        "/": (-1, 9),
        "square": 9,
        "cube": 9,
        "exp": 9,
    },
    # ^ Limit the complexity within each argument.
    # "inv": (-1, 9) states that the numerator has no constraint,
    # but the denominator has a max complexity of 9.
    # "exp": 9 simply states that `exp` can only have
    # an expression of complexity 9 as input.
    nested_constraints={
        "square": {"square": 1, "cube": 1, "exp": 0},
        "cube": {"square": 1, "cube": 1, "exp": 0},
        "exp": {"square": 1, "cube": 1, "exp": 0},
    },
    # ^ Nesting constraints on operators. For example,
    # "square(exp(x))" is not allowed, since "square": {"exp": 0}.


 weight_randomize=0.1,

 cluster_manager="slurm",
 precision=64


DSR
max epoch can be set
From 2204.10532 section "Training" we see that
2204.10532We optimize a cross-entropy loss with the Adam optimizer, warming up the learning rate from 1e−7 to 2.1e−4 over the first 10,000 steps, then decaying it as the inverse square root of the number of steps, following [23]. We ... train
our models until the accuracy on the validation set saturates (around 50 epochs of 3M examples).
Bottom of page 6: The model works best if data is randomsly split into bags of datasize 200.
They don't themselves seem to vary anything except number of datapoints, number of unary operators and binary operators (see beginning of section 3.1). I'd say we should keep these things fixed though...Hence all we do here is choose the appropriate operators (see below) and the appropriate number of max epochs (based on what we choose for other algorithms).

In symbolicregression/symbolicregression/regressors.py around line 100 we see the possible functions from which we should choose
            'add': lambda x, y : x + y,
            'sub': lambda x, y : x - y,
            'mul': lambda x, y : x*y,
            'div': lambda x, y : x/y,
            'sqrt': lambda x : x**0.5,
            'log': lambda x : log(x),
            'neg': lambda x : -x,
            'inv': lambda x : 1/x,
            'sin': lambda x : sin(x),
            'cos': lambda x : cos(x),
            'pow': lambda x, y : x**y
